Demystifying Privacy in 5G Stand Alone Networks

Ensuring user privacy remains critical in mobile networks, particularly with the rise of connected devices and denser 5G infrastructure. Privacy concerns have persisted across 2G, 3G, and 4G/LTE networks. Recognizing these concerns, the 3rd Generation Partnership Project (3GPP) has made privacy enhancements in 5G Release 15. However, the extent of operator adoption remains unclear, especially as most networks operate in 5G Non Stand Alone (NSA) mode, relying on 4G Core Networks. This study provides the first qualitative and experimental comparison between 5G NSA and Stand Alone (SA) in real operator networks, focusing on privacy enhancements addressing top eight pre-5G attacks based on recent academic literature. Additionally, it evaluates the privacy levels of OpenAirInterface (OAI), a leading open-source software for 5G, against real network deployments for the same attacks. The analysis reveals two new 5G privacy vulnerabilities, underscoring the need for further research and stricter standards.

==> main <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{97}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[suc(2021)]%
        {suci_related_solutions}
 \bibinfo{year}{2021}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 33.846, “Study on authentication
  enhancements in the 5G System (5GS),” version 17.0.0 Rel. 17}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[gr-(2021)]%
        {gr-LTE}
 \bibinfo{year}{2021}\natexlab{}.
\newblock \bibinfo{title}{{gr-LTE: GNU Radio LTE receiver}}.
\newblock \bibinfo{howpublished}{\url{https://github.com/kit-cel/gr-lte/}}.
\newblock
\newblock
\shownote{Accessed 2024-02}.


\bibitem[Ope(2021)]%
        {OpenLTE}
 \bibinfo{year}{2021}\natexlab{}.
\newblock \bibinfo{title}{{OpenLTE: An open source 3GPP LTE implementation}}.
\newblock
  \bibinfo{howpublished}{\url{https://sourceforge.net/projects/openlte/}}.
\newblock
\newblock
\shownote{Accessed 2024-02}.


\bibitem[Num(2023)]%
        {Numbering}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 23.003, “Numbering, addressing and
  identification,” version 18.2.0 Rel. 18}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[5GS(2023)]%
        {5GS_architecture}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 23.501, “System architecture for the 5G
  System (5GS),” version 18.3.0 Rel. 18}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3GP(2023)]%
        {3GPP_NAS}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 24.501, “Non-Access-Stratum (NAS) protocol
  for 5G System (5GS),” version 18.4.0 Rel. 18}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3g_(2023)]%
        {3g_security}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 33.102, “3G Security; Security
  Architecture,” version 17.0.0 Rel. 17}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3gp(2023a)]%
        {3gpp_IMSI_catching_problem}
 \bibinfo{year}{2023}\natexlab{a}.
\newblock \bibinfo{title}{{3GPP TS 33.401, “3GPP System Architecture
  Evolution (SAE); Security architecture,” version 17.4.0 Rel. 17}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3gp(2023b)]%
        {3gpp_fake_base_stations}
 \bibinfo{year}{2023}\natexlab{b}.
\newblock \bibinfo{title}{{3GPP TS 33.501, “Security architecture and
  procedures for 5G system,” version 18.2.0 Rel. 18}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[ims(2023)]%
        {imsiProbing3GPP}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{3GPP TS 33.846, “Study on authentication
  enhancements in the 5G System (5GS),” version 17.0.0 Rel. 17}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3GP(2023a)]%
        {3GPP_Radio_Access_Capab}
 \bibinfo{year}{2023}\natexlab{a}.
\newblock \bibinfo{title}{{3GPP TS 38.306, “NR; User Equipment (UE) radio
  access capabilities,” version 18.0.0 Rel. 18}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[3GP(2023b)]%
        {3GPP_RRC}
 \bibinfo{year}{2023}\natexlab{b}.
\newblock \bibinfo{title}{{3GPP TS 38.331, “NR; Radio Resource Control (RRC)
  protocol specification,” version 17.6.0 Rel. 17}}.
\newblock \bibinfo{howpublished}{\url{https://www.3gpp.org/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[srs(2023)]%
        {srsRAN}
 \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{srsRAN: an open source 4G software radio suite
  developed by SRS}}.
\newblock \bibinfo{howpublished}{\url{https://github.com/srsran/srsRAN_4G/}}.
\newblock
\newblock
\shownote{Accessed 2024-02}.


\bibitem[USR(2024)]%
        {USRP}
 \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{{Ettus. USRP.}}
\newblock \bibinfo{howpublished}{\url{https://www.ettus.com/products/}}.
\newblock
\newblock
\shownote{Accessed 2024-02}.


\bibitem[OAI(2024)]%
        {OAI}
 \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{{OpenAirInterface Source Code for Next Generation
  Cellular Standard}}.
\newblock \bibinfo{howpublished}{\url{https://gitlab.eurecom.fr/oai/}}.
\newblock
\newblock
\shownote{Accessed 2024-02}.


\bibitem[Mes(tion)]%
        {MessengerApp}
 \bibinfo{year}{Messenger application}\natexlab{}.
\newblock \bibinfo{title}{{2024}}.
\newblock \bibinfo{howpublished}{\url{https://www.messenger.com/}}.
\newblock
\newblock
\shownote{Accessed: 03-2024}.


\bibitem[Nem(tion)]%
        {NemoHandy}
 \bibinfo{year}{Nemo Handy Handheld Measurement Solution}\natexlab{}.
\newblock \bibinfo{title}{{2024}}.
\newblock
  \bibinfo{howpublished}{\url{https://www.keysight.com/us/en/product/NTH50047B/nemo-handy-handheld-measurement-solution.html/}}.
\newblock
\newblock
\shownote{Accessed: 03-2024}.


\bibitem[sta(2030)]%
        {statistic_IoT_devices}
 \bibinfo{year}{Number of Internet of Things (IoT) connected devices worldwide
  from 2019 to 2023, with forecasts from 2022 to 2030}\natexlab{}.
\newblock \bibinfo{title}{{2023}}.
\newblock
  \bibinfo{howpublished}{\url{https://www.statista.com/statistics/1183457/iot-connected-devices-worldwide//}}.
\newblock
\newblock
\shownote{Accessed: 03-2024}.


\bibitem[5GAmericas(2023)]%
        {5gamericas}
\bibfield{author}{\bibinfo{person}{5GAmericas}.}
  \bibinfo{year}{2023}\natexlab{}.
\newblock \bibinfo{title}{{Global 5G Connections Increase 76\% Annually and Now
  Reaches 1.05 Billion}}.
\newblock
  \bibinfo{howpublished}{\url{https://www.5gamericas.org/global-5g-connections-increase-76-annually-and-now-reaches-1-05-billion/}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[Ahmadian et~al\mbox{.}(2009)]%
        {ahmadian2009new}
\bibfield{author}{\bibinfo{person}{Zahra Ahmadian}, \bibinfo{person}{Somayeh
  Salimi}, {and} \bibinfo{person}{Ahmad Salahi}.}
  \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{{New attacks on UMTS network access}}. In
  \bibinfo{booktitle}{\emph{2009 Wireless Telecommunications Symposium}}. IEEE,
  \bibinfo{pages}{1--6}.
\newblock


\bibitem[Arapinis et~al\mbox{.}(2012)]%
        {arapinis2012new}
\bibfield{author}{\bibinfo{person}{Myrto Arapinis}, \bibinfo{person}{Loretta
  Mancini}, \bibinfo{person}{Eike Ritter}, \bibinfo{person}{Mark Ryan},
  \bibinfo{person}{Nico Golde}, \bibinfo{person}{Kevin Redon}, {and}
  \bibinfo{person}{Ravishankar Borgaonkar}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{New privacy issues in mobile telephony: fix and
  verification}}. In \bibinfo{booktitle}{\emph{Proceedings of the 2012 ACM
  conference on Computer and communications security}}.
  \bibinfo{pages}{205--216}.
\newblock


\bibitem[Arapinis et~al\mbox{.}(2014)]%
        {arapinis2014privacy}
\bibfield{author}{\bibinfo{person}{Myrto Arapinis},
  \bibinfo{person}{Loretta~Ilaria Mancini}, \bibinfo{person}{Eike Ritter},
  {and} \bibinfo{person}{Mark Ryan}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{Privacy through Pseudonymity in Mobile Telephony
  Systems.}}. In \bibinfo{booktitle}{\emph{NDSS}}.
\newblock


\bibitem[Arapinis et~al\mbox{.}(2017)]%
        {arapinis2017analysis}
\bibfield{author}{\bibinfo{person}{Myrto Arapinis},
  \bibinfo{person}{Loretta~Ilaria Mancini}, \bibinfo{person}{Eike Ritter},
  {and} \bibinfo{person}{Mark~Dermot Ryan}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Analysis of privacy in mobile telephony systems}}.
\newblock \bibinfo{journal}{\emph{International Journal of Information
  Security}}  \bibinfo{volume}{16} (\bibinfo{year}{2017}),
  \bibinfo{pages}{491--523}.
\newblock


\bibitem[Basin et~al\mbox{.}(2018)]%
        {basin2018formal}
\bibfield{author}{\bibinfo{person}{David Basin}, \bibinfo{person}{Jannik
  Dreier}, \bibinfo{person}{Lucca Hirschi}, \bibinfo{person}{Sa{\v{s}}a
  Radomirovic}, \bibinfo{person}{Ralf Sasse}, {and} \bibinfo{person}{Vincent
  Stettler}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{A formal analysis of 5G authentication}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2018 ACM SIGSAC conference on
  computer and communications security}}. \bibinfo{pages}{1383--1396}.
\newblock


\bibitem[Behrad et~al\mbox{.}(2018)]%
        {behrad2018securing}
\bibfield{author}{\bibinfo{person}{Shanay Behrad}, \bibinfo{person}{Emmanuel
  Bertin}, {and} \bibinfo{person}{Noel Crespi}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Securing authentication for mobile networks, a
  survey on 4G issues and 5G answers}}. In \bibinfo{booktitle}{\emph{2018 21st
  conference on innovation in clouds, internet and networks and workshops
  (ICIN)}}. IEEE, \bibinfo{pages}{1--8}.
\newblock


\bibitem[Bitsikas and P{\"o}pper(2021)]%
        {bitsikas2021don}
\bibfield{author}{\bibinfo{person}{Evangelos Bitsikas} {and}
  \bibinfo{person}{Christina P{\"o}pper}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{Don’t hand it over: Vulnerabilities in the
  handover procedure of cellular telecommunications}}. In
  \bibinfo{booktitle}{\emph{Annual Computer Security Applications Conference}}.
  \bibinfo{pages}{900--915}.
\newblock


\bibitem[Bojic et~al\mbox{.}(2017)]%
        {bojic2017opportunities}
\bibfield{author}{\bibinfo{person}{Iva Bojic}, \bibinfo{person}{Yuji
  Yoshimura}, {and} \bibinfo{person}{Carlo Ratti}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Opportunities and challenges of trip generation
  data collection techniques using cellular networks}}.
\newblock \bibinfo{journal}{\emph{IEEE Communications Magazine}}
  \bibinfo{volume}{55}, \bibinfo{number}{3} (\bibinfo{year}{2017}),
  \bibinfo{pages}{204--209}.
\newblock


\bibitem[Borgaonkar et~al\mbox{.}(2018)]%
        {borgaonkar2018new}
\bibfield{author}{\bibinfo{person}{Ravishankar Borgaonkar},
  \bibinfo{person}{Lucca Hirschi}, \bibinfo{person}{Shinjo Park}, {and}
  \bibinfo{person}{Altaf Shaik}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{New privacy threat on 3G, 4G, and upcoming 5G AKA
  protocols}}.
\newblock \bibinfo{journal}{\emph{Cryptology ePrint Archive}}
  (\bibinfo{year}{2018}).
\newblock


\bibitem[Bui and Widmer(2016)]%
        {bui2016owl}
\bibfield{author}{\bibinfo{person}{Nicola Bui} {and} \bibinfo{person}{Joerg
  Widmer}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{OWL: A reliable online watcher for LTE control
  channel measurements}}. In \bibinfo{booktitle}{\emph{Proceedings of the 5th
  Workshop on All Things Cellular: Operations, Applications and Challenges}}.
  \bibinfo{pages}{25--30}.
\newblock


\bibitem[Chlosta et~al\mbox{.}(2019)]%
        {chlosta2019lte}
\bibfield{author}{\bibinfo{person}{Merlin Chlosta}, \bibinfo{person}{David
  Rupprecht}, \bibinfo{person}{Thorsten Holz}, {and} \bibinfo{person}{Christina
  P{\"o}pper}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{LTE security disabled: misconfiguration in
  commercial networks}}. In \bibinfo{booktitle}{\emph{Proceedings of the 12th
  conference on security and privacy in wireless and mobile networks}}.
  \bibinfo{pages}{261--266}.
\newblock


\bibitem[Chlosta et~al\mbox{.}(2021)]%
        {chlosta20215g}
\bibfield{author}{\bibinfo{person}{Merlin Chlosta}, \bibinfo{person}{David
  Rupprecht}, \bibinfo{person}{Christina P{\"o}pper}, {and}
  \bibinfo{person}{Thorsten Holz}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{5G SUCI-Catchers: Still catching them all?}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 14th ACM Conference on Security
  and Privacy in Wireless and Mobile Networks}}. \bibinfo{pages}{359--364}.
\newblock


\bibitem[Choudhury et~al\mbox{.}(2012)]%
        {choudhury2012enhancing}
\bibfield{author}{\bibinfo{person}{Hiten Choudhury}, \bibinfo{person}{Basav
  Roychoudhury}, {and} \bibinfo{person}{Dilip~Kr Saikia}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Enhancing user identity privacy in LTE}}. In
  \bibinfo{booktitle}{\emph{2012 IEEE 11th International Conference on Trust,
  Security and Privacy in Computing and Communications}}. IEEE,
  \bibinfo{pages}{949--957}.
\newblock


\bibitem[Dabrowski et~al\mbox{.}(2016)]%
        {dabrowski2016messenger}
\bibfield{author}{\bibinfo{person}{Adrian Dabrowski}, \bibinfo{person}{Georg
  Petzl}, {and} \bibinfo{person}{Edgar~R Weippl}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{The messenger shoots back: Network operator based
  IMSI catcher detection}}. In \bibinfo{booktitle}{\emph{Research in Attacks,
  Intrusions, and Defenses: 19th International Symposium, RAID 2016, Paris,
  France, September 19-21, 2016, Proceedings 19}}. Springer,
  \bibinfo{pages}{279--302}.
\newblock


\bibitem[Dabrowski et~al\mbox{.}(2014)]%
        {dabrowski2014imsi}
\bibfield{author}{\bibinfo{person}{Adrian Dabrowski}, \bibinfo{person}{Nicola
  Pianta}, \bibinfo{person}{Thomas Klepp}, \bibinfo{person}{Martin Mulazzani},
  {and} \bibinfo{person}{Edgar Weippl}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{IMSI-catch me if you can: IMSI-catcher-catchers}}.
  In \bibinfo{booktitle}{\emph{Proceedings of the 30th annual computer security
  applications Conference}}. \bibinfo{pages}{246--255}.
\newblock


\bibitem[Demel et~al\mbox{.}(2015)]%
        {demel2015lte}
\bibfield{author}{\bibinfo{person}{Johannes Demel}, \bibinfo{person}{Sebastian
  Koslowski}, {and} \bibinfo{person}{Friedrich~K Jondral}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{{A LTE receiver framework using GNU Radio}}.
\newblock \bibinfo{journal}{\emph{Journal of Signal Processing Systems}}
  \bibinfo{volume}{78} (\bibinfo{year}{2015}), \bibinfo{pages}{313--320}.
\newblock


\bibitem[Deng et~al\mbox{.}(2009)]%
        {deng2009novel}
\bibfield{author}{\bibinfo{person}{Yaping Deng}, \bibinfo{person}{Hong Fu},
  \bibinfo{person}{Xianzhong Xie}, \bibinfo{person}{Jihua Zhou},
  \bibinfo{person}{Yucheng Zhang}, {and} \bibinfo{person}{Jinling Shi}.}
  \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{{A novel 3GPP SAE authentication and key agreement
  protocol}}. In \bibinfo{booktitle}{\emph{2009 IEEE International Conference
  on Network Infrastructure and Digital Content}}. IEEE,
  \bibinfo{pages}{557--561}.
\newblock


\bibitem[Ekene et~al\mbox{.}(2016)]%
        {ekene2016enhanced}
\bibfield{author}{\bibinfo{person}{Okoye~Emmanuel Ekene}, \bibinfo{person}{Ron
  Ruhl}, {and} \bibinfo{person}{Pavol Zavarsky}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Enhanced user security and privacy protection in
  4G LTE network}}. In \bibinfo{booktitle}{\emph{2016 IEEE 40th Annual Computer
  Software and Applications Conference (COMPSAC)}}, Vol.~\bibinfo{volume}{2}.
  IEEE, \bibinfo{pages}{443--448}.
\newblock


\bibitem[Eleftherakis et~al\mbox{.}(2024)]%
        {eleftherakis2024sokevaluating5gprotocols}
\bibfield{author}{\bibinfo{person}{Stavros Eleftherakis},
  \bibinfo{person}{Domenico Giustiniano}, {and} \bibinfo{person}{Nicolas
  Kourtellis}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{{SoK: Evaluating 5G Protocols Against Legacy and
  Emerging Privacy and Security Attacks}}.
\newblock
\newblock
\showeprint[arxiv]{2409.06360}~[cs.CR]
\urldef\tempurl%
\url{https://arxiv.org/abs/2409.06360}
\showURL{%
\tempurl}


\bibitem[Erni et~al\mbox{.}(2022)]%
        {erni2022adaptover}
\bibfield{author}{\bibinfo{person}{Simon Erni}, \bibinfo{person}{Martin
  Kotuliak}, \bibinfo{person}{Patrick Leu}, \bibinfo{person}{Marc Roeschlin},
  {and} \bibinfo{person}{Srdjan Capkun}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{{AdaptOver: adaptive overshadowing attacks in
  cellular networks}}. In \bibinfo{booktitle}{\emph{Proceedings of the 28th
  Annual International Conference on Mobile Computing And Networking}}.
  \bibinfo{pages}{743--755}.
\newblock


\bibitem[Falkenberg and Wietfeld(2019)]%
        {falkenberg2019falcon}
\bibfield{author}{\bibinfo{person}{Robert Falkenberg} {and}
  \bibinfo{person}{Christian Wietfeld}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{FALCON: An accurate real-time monitor for
  client-based mobile network data analytics}}. In
  \bibinfo{booktitle}{\emph{2019 IEEE Global Communications Conference
  (GLOBECOM)}}. IEEE, \bibinfo{pages}{1--7}.
\newblock


\bibitem[Fei and Wang(2023)]%
        {fei2023vulnerability}
\bibfield{author}{\bibinfo{person}{Teng Fei} {and} \bibinfo{person}{Wenye
  Wang}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{{The vulnerability and enhancement of AKA protocol
  for mobile authentication in LTE/5G networks}}.
\newblock \bibinfo{journal}{\emph{Computer Networks}}  \bibinfo{volume}{228}
  (\bibinfo{year}{2023}), \bibinfo{pages}{109685}.
\newblock


\bibitem[Frick and Bott(2000)]%
        {patent}
\bibfield{author}{\bibinfo{person}{Joachim Frick} {and} \bibinfo{person}{Rainer
  Bott}.} \bibinfo{year}{2000}\natexlab{}.
\newblock \bibinfo{title}{{Method for identifying a mobile phone user or for
  eavesdropping on outgoing calls}}.
\newblock
\newblock
\newblock
\shownote{Patent, Rohde \& Schwarz, EP 1051053}.


\bibitem[Geir et~al\mbox{.}(2013)]%
        {geir2013privacy}
\bibfield{author}{\bibinfo{person}{M~K{\o}ien Geir} {et~al\mbox{.}}}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{{Privacy enhanced mutual authentication in LTE}}.
  In \bibinfo{booktitle}{\emph{2013 IEEE 9th International Conference on
  Wireless and Mobile Computing, Networking and Communications (WiMob)}}. IEEE,
  \bibinfo{pages}{614--621}.
\newblock


\bibitem[Gomez-Miguelez et~al\mbox{.}(2016)]%
        {gomez2016srslte}
\bibfield{author}{\bibinfo{person}{Ismael Gomez-Miguelez},
  \bibinfo{person}{Andres Garcia-Saavedra}, \bibinfo{person}{Paul~D Sutton},
  \bibinfo{person}{Pablo Serrano}, \bibinfo{person}{Cristina Cano}, {and}
  \bibinfo{person}{Doug~J Leith}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{srsLTE: An open-source platform for LTE evolution
  and experimentation}}. In \bibinfo{booktitle}{\emph{Proceedings of the Tenth
  ACM International Workshop on Wireless Network Testbeds, Experimental
  Evaluation, and Characterization}}. \bibinfo{pages}{25--32}.
\newblock


\bibitem[Hahn et~al\mbox{.}(2014)]%
        {hahn2014privacy}
\bibfield{author}{\bibinfo{person}{Changhee Hahn}, \bibinfo{person}{Hyunsoo
  Kwon}, \bibinfo{person}{Daeyoung Kim}, \bibinfo{person}{Kyungtae Kang}, {and}
  \bibinfo{person}{Junbeom Hur}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{A privacy threat in 4th generation mobile
  telephony and its countermeasure}}. In \bibinfo{booktitle}{\emph{Wireless
  Algorithms, Systems, and Applications: 9th International Conference, WASA
  2014, Harbin, China, June 23-25, 2014. Proceedings 9}}. Springer,
  \bibinfo{pages}{624--635}.
\newblock


\bibitem[Hoang et~al\mbox{.}(2023)]%
        {hoang2023ltesniffer}
\bibfield{author}{\bibinfo{person}{Tuan~Dinh Hoang}, \bibinfo{person}{CheolJun
  Park}, \bibinfo{person}{Mincheol Son}, \bibinfo{person}{Taekkyung Oh},
  \bibinfo{person}{Sangwook Bae}, \bibinfo{person}{Junho Ahn},
  \bibinfo{person}{Beomseok Oh}, {and} \bibinfo{person}{Yongdae Kim}.}
  \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{{LTESniffer: An Open-source LTE Downlink/Uplink
  Eavesdropper}}.
\newblock  (\bibinfo{year}{2023}).
\newblock


\bibitem[Hong et~al\mbox{.}(2018)]%
        {hong2018guti}
\bibfield{author}{\bibinfo{person}{Byeongdo Hong}, \bibinfo{person}{Sangwook
  Bae}, {and} \bibinfo{person}{Yongdae Kim}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{GUTI Reallocation Demystified: Cellular Location
  Tracking with Changing Temporary Identifier.}}. In
  \bibinfo{booktitle}{\emph{NDSS}}.
\newblock


\bibitem[Hussain et~al\mbox{.}(2018)]%
        {hussain2018lteinspector}
\bibfield{author}{\bibinfo{person}{Syed Hussain}, \bibinfo{person}{Omar
  Chowdhury}, \bibinfo{person}{Shagufta Mehnaz}, {and} \bibinfo{person}{Elisa
  Bertino}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{LTEInspector: A systematic approach for
  adversarial testing of 4G LTE}}. In \bibinfo{booktitle}{\emph{Network and
  Distributed Systems Security (NDSS) Symposium 2018}}.
\newblock


\bibitem[Hussain et~al\mbox{.}(2019a)]%
        {hussain2019privacy}
\bibfield{author}{\bibinfo{person}{Syed~Rafiul Hussain},
  \bibinfo{person}{Mitziu Echeverria}, \bibinfo{person}{Omar Chowdhury},
  \bibinfo{person}{Ninghui Li}, {and} \bibinfo{person}{Elisa Bertino}.}
  \bibinfo{year}{2019}\natexlab{a}.
\newblock \showarticletitle{{Privacy attacks to the 4G and 5G cellular paging
  protocols using side channel information}}.
\newblock \bibinfo{journal}{\emph{Network and distributed systems security
  (NDSS) symposium2019}} (\bibinfo{year}{2019}).
\newblock


\bibitem[Hussain et~al\mbox{.}(2019b)]%
        {hussain20195greasoner}
\bibfield{author}{\bibinfo{person}{Syed~Rafiul Hussain},
  \bibinfo{person}{Mitziu Echeverria}, \bibinfo{person}{Imtiaz Karim},
  \bibinfo{person}{Omar Chowdhury}, {and} \bibinfo{person}{Elisa Bertino}.}
  \bibinfo{year}{2019}\natexlab{b}.
\newblock \showarticletitle{{5GReasoner: A property-directed security and
  privacy analysis framework for 5G cellular network protocol}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2019 ACM SIGSAC Conference on
  Computer and Communications Security}}. \bibinfo{pages}{669--684}.
\newblock


\bibitem[Jover(2016a)]%
        {jover2016lte_first}
\bibfield{author}{\bibinfo{person}{Roger~Piqueras Jover}.}
  \bibinfo{year}{2016}\natexlab{a}.
\newblock \showarticletitle{{LTE security and protocol exploits}}.
\newblock \bibinfo{journal}{\emph{Shmoocon 2016}} (\bibinfo{year}{2016}).
\newblock


\bibitem[Jover(2016b)]%
        {jover2016lte}
\bibfield{author}{\bibinfo{person}{Roger~Piqueras Jover}.}
  \bibinfo{year}{2016}\natexlab{b}.
\newblock \showarticletitle{{LTE security, protocol exploits and location
  tracking experimentation with low-cost software radio}}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1607.05171}}
  (\bibinfo{year}{2016}).
\newblock


\bibitem[Karakoc et~al\mbox{.}(2023)]%
        {karakoc2023never}
\bibfield{author}{\bibinfo{person}{Bedran Karakoc}, \bibinfo{person}{Nils
  F{\"u}rste}, \bibinfo{person}{David Rupprecht}, {and}
  \bibinfo{person}{Katharina Kohls}.} \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{{Never Let Me Down Again: Bidding-Down Attacks and
  Mitigations in 5G and 4G}}.
\newblock  (\bibinfo{year}{2023}).
\newblock


\bibitem[Khan et~al\mbox{.}(2018)]%
        {khan2018identity}
\bibfield{author}{\bibinfo{person}{Haibat Khan}, \bibinfo{person}{Benjamin
  Dowling}, {and} \bibinfo{person}{Keith~M Martin}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Identity confidentiality in 5G mobile telephony
  systems}}. In \bibinfo{booktitle}{\emph{International Conference on Research
  in Security Standardisation}}. Springer, \bibinfo{pages}{120--142}.
\newblock


\bibitem[Khan and Martin(2020)]%
        {khan2020survey}
\bibfield{author}{\bibinfo{person}{Haibat Khan} {and} \bibinfo{person}{Keith~M
  Martin}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{{A survey of subscription privacy on the 5G radio
  interface-the past, present and future}}.
\newblock \bibinfo{journal}{\emph{Journal of Information Security and
  Applications}}  \bibinfo{volume}{53} (\bibinfo{year}{2020}),
  \bibinfo{pages}{102537}.
\newblock


\bibitem[Khan and Mitchell(2014)]%
        {khan2014another}
\bibfield{author}{\bibinfo{person}{Mohammed Shafiul~Alam Khan} {and}
  \bibinfo{person}{Chris~J Mitchell}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{Another look at privacy threats in 3G mobile
  telephony}}. In \bibinfo{booktitle}{\emph{Australasian Conference on
  Information Security and Privacy}}. Springer, \bibinfo{pages}{386--396}.
\newblock


\bibitem[Khan and Mitchell(2015)]%
        {khan2015improving}
\bibfield{author}{\bibinfo{person}{Mohammed Shafiul~Alam Khan} {and}
  \bibinfo{person}{Chris~J Mitchell}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{{Improving air interface user privacy in mobile
  telephony}}. In \bibinfo{booktitle}{\emph{Security Standardisation Research:
  Second International Conference, SSR 2015, Tokyo, Japan, December 15-16,
  2015, Proceedings 2}}. Springer, \bibinfo{pages}{165--184}.
\newblock


\bibitem[Khan and Mitchell(2017)]%
        {khan2017trashing}
\bibfield{author}{\bibinfo{person}{Mohammed Shafiul~Alam Khan} {and}
  \bibinfo{person}{Chris~J Mitchell}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Trashing IMSI catchers in mobile networks}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 10th ACM Conference on Security
  and Privacy in Wireless and Mobile Networks}}. \bibinfo{pages}{207--218}.
\newblock


\bibitem[Khan et~al\mbox{.}(2019)]%
        {khan2019survey}
\bibfield{author}{\bibinfo{person}{Rabia Khan}, \bibinfo{person}{Pardeep
  Kumar}, \bibinfo{person}{Dushantha Nalin~K Jayakody}, {and}
  \bibinfo{person}{Madhusanka Liyanage}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{A survey on security and privacy of 5G
  technologies: Potential solutions, recent advancements, and future
  directions}}.
\newblock \bibinfo{journal}{\emph{IEEE Communications Surveys \& Tutorials}}
  \bibinfo{volume}{22}, \bibinfo{number}{1} (\bibinfo{year}{2019}),
  \bibinfo{pages}{196--248}.
\newblock


\bibitem[Kohls et~al\mbox{.}(2019)]%
        {kohls2019lost}
\bibfield{author}{\bibinfo{person}{Katharina Kohls}, \bibinfo{person}{David
  Rupprecht}, \bibinfo{person}{Thorsten Holz}, {and} \bibinfo{person}{Christina
  P{\"o}pper}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{Lost traffic encryption: fingerprinting LTE/4G
  traffic on layer two}}. In \bibinfo{booktitle}{\emph{Proceedings of the 12th
  Conference on Security and Privacy in Wireless and Mobile Networks}}.
  \bibinfo{pages}{249--260}.
\newblock


\bibitem[Kotuliak et~al\mbox{.}(2022)]%
        {kotuliak2022ltrack}
\bibfield{author}{\bibinfo{person}{Martin Kotuliak}, \bibinfo{person}{Simon
  Erni}, \bibinfo{person}{Patrick Leu}, \bibinfo{person}{Marc R{\"o}schlin},
  {and} \bibinfo{person}{Srdjan {\v{C}}apkun}.}
  \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{$\{$LTrack$\}$: Stealthy tracking of mobile phones
  in $\{$LTE$\}$}. In \bibinfo{booktitle}{\emph{31st USENIX Security Symposium
  (USENIX Security 22)}}. \bibinfo{pages}{1291--1306}.
\newblock


\bibitem[Koutsos(2019)]%
        {koutsos20195g}
\bibfield{author}{\bibinfo{person}{Adrien Koutsos}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{The 5G-AKA authentication protocol privacy}}. In
  \bibinfo{booktitle}{\emph{2019 IEEE European symposium on security and
  privacy (EuroS\&P)}}. IEEE, \bibinfo{pages}{464--479}.
\newblock


\bibitem[Kumar et~al\mbox{.}(2014)]%
        {kumar2014lte}
\bibfield{author}{\bibinfo{person}{Swarun Kumar}, \bibinfo{person}{Ezzeldin
  Hamed}, \bibinfo{person}{Dina Katabi}, {and} \bibinfo{person}{Li Erran~Li}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{LTE radio analytics made easy and accessible}}.
\newblock \bibinfo{journal}{\emph{ACM SIGCOMM Computer Communication Review}}
  \bibinfo{volume}{44}, \bibinfo{number}{4} (\bibinfo{year}{2014}),
  \bibinfo{pages}{211--222}.
\newblock


\bibitem[Kune et~al\mbox{.}(2012)]%
        {kune2012location}
\bibfield{author}{\bibinfo{person}{Denis~Foo Kune}, \bibinfo{person}{John
  Koelndorfer}, \bibinfo{person}{Nicholas Hopper}, {and}
  \bibinfo{person}{Yongdae Kim}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Location leaks on the GSM air interface}}.
\newblock \bibinfo{journal}{\emph{ISOC NDSS (Feb 2012)}}
  (\bibinfo{year}{2012}).
\newblock


\bibitem[Lasierra et~al\mbox{.}(2023)]%
        {lasierra2023european}
\bibfield{author}{\bibinfo{person}{Oscar Lasierra}, \bibinfo{person}{Gines
  Garcia-Aviles}, \bibinfo{person}{Esteban Municio}, \bibinfo{person}{Antonio
  Skarmeta}, {and} \bibinfo{person}{Xavier Costa-P{\'e}rez}.}
  \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{{European 5G Security in the Wild: Reality versus
  Expectations}}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2305.08635}}
  (\bibinfo{year}{2023}).
\newblock


\bibitem[Li and Wang(2011)]%
        {li2011security}
\bibfield{author}{\bibinfo{person}{Xiehua Li} {and} \bibinfo{person}{Yongjun
  Wang}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Security enhanced authentication and key agreement
  protocol for LTE/SAE network}}. In \bibinfo{booktitle}{\emph{2011 7th
  International Conference on Wireless Communications, Networking and Mobile
  Computing}}. IEEE, \bibinfo{pages}{1--4}.
\newblock


\bibitem[Lilly(2017)]%
        {lilly2017imsi}
\bibfield{author}{\bibinfo{person}{Andy Lilly}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{IMSI catchers: hacking mobile communications}}.
\newblock \bibinfo{journal}{\emph{Network Security}} \bibinfo{volume}{2017},
  \bibinfo{number}{2} (\bibinfo{year}{2017}), \bibinfo{pages}{5--7}.
\newblock


\bibitem[Liu et~al\mbox{.}(2021)]%
        {liu2021security}
\bibfield{author}{\bibinfo{person}{Fuwen Liu}, \bibinfo{person}{Li Su},
  \bibinfo{person}{Bo Yang}, \bibinfo{person}{Haitao Du},
  \bibinfo{person}{Minpeng Qi}, {and} \bibinfo{person}{Shen He}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{Security Enhancements to Subscriber Privacy
  Protection Scheme in 5G Systems}}. In \bibinfo{booktitle}{\emph{2021
  International Wireless Communications and Mobile Computing (IWCMC)}}. IEEE,
  \bibinfo{pages}{451--456}.
\newblock


\bibitem[Ludant and Noubir(2021)]%
        {ludant2021sigunder}
\bibfield{author}{\bibinfo{person}{Norbert Ludant} {and}
  \bibinfo{person}{Guevara Noubir}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{SigUnder: a stealthy 5G low power attack and
  defenses}}. In \bibinfo{booktitle}{\emph{Proceedings of the 14th ACM
  Conference on Security and Privacy in Wireless and Mobile Networks}}.
  \bibinfo{pages}{250--260}.
\newblock


\bibitem[Ludant et~al\mbox{.}(2023)]%
        {ludant20235g}
\bibfield{author}{\bibinfo{person}{Norbert Ludant}, \bibinfo{person}{Pieter
  Robyns}, {and} \bibinfo{person}{Guevara Noubir}.}
  \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{{From 5G Sniffing to Harvesting Leakages of
  Privacy-Preserving Messengers}}. In \bibinfo{booktitle}{\emph{2023 IEEE
  Symposium on Security and Privacy (SP)}}. IEEE, \bibinfo{pages}{3146--3161}.
\newblock


\bibitem[Marsden and Marshall(2014)]%
        {multipleIMSIs}
\bibfield{author}{\bibinfo{person}{Ian Marsden} {and} \bibinfo{person}{Paul
  Marshall}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \bibinfo{title}{{Multi IMSI system and method}}.
\newblock
\newblock
\newblock
\shownote{US Patent App. 13/966,350}.


\bibitem[Meyer and Wetzel(2004)]%
        {meyer2004man}
\bibfield{author}{\bibinfo{person}{Ulrike Meyer} {and} \bibinfo{person}{Susanne
  Wetzel}.} \bibinfo{year}{2004}\natexlab{}.
\newblock \showarticletitle{{A man-in-the-middle attack on UMTS}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 3rd ACM workshop on Wireless
  security}}. \bibinfo{pages}{90--97}.
\newblock


\bibitem[Michau and Devine(2016)]%
        {michau2016not}
\bibfield{author}{\bibinfo{person}{Benoit Michau} {and}
  \bibinfo{person}{Christophe Devine}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{How to not break LTE crypto}}. In
  \bibinfo{booktitle}{\emph{ANSSI Symposium sur la s{\'e}curit{\'e} des
  technologies de l’information et des communications (SSTIC)}}.
\newblock


\bibitem[Mitchell(2001)]%
        {mitchell2001security}
\bibfield{author}{\bibinfo{person}{Chris Mitchell}.}
  \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{{The security of the GSM air interface protocol}}.
\newblock \bibinfo{journal}{\emph{Univ. of London, Royal Holloway,
  RHUL-MA-2001-3}} (\bibinfo{year}{2001}).
\newblock


\bibitem[Nie et~al\mbox{.}(2022)]%
        {nie2022measuring}
\bibfield{author}{\bibinfo{person}{Shiyue Nie}, \bibinfo{person}{Yiming Zhang},
  \bibinfo{person}{Tao Wan}, \bibinfo{person}{Haixin Duan}, {and}
  \bibinfo{person}{Song Li}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{{Measuring the deployment of 5g security
  enhancement}}. In \bibinfo{booktitle}{\emph{Proceedings of the 15th ACM
  Conference on Security and Privacy in Wireless and Mobile Networks}}.
  \bibinfo{pages}{169--174}.
\newblock


\bibitem[Nikaein et~al\mbox{.}(2014)]%
        {nikaein2014openairinterface}
\bibfield{author}{\bibinfo{person}{Navid Nikaein}, \bibinfo{person}{Mahesh~K
  Marina}, \bibinfo{person}{Saravana Manickam}, \bibinfo{person}{Alex Dawson},
  \bibinfo{person}{Raymond Knopp}, {and} \bibinfo{person}{Christian Bonnet}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{OpenAirInterface: A flexible platform for 5G
  research}}.
\newblock \bibinfo{journal}{\emph{ACM SIGCOMM Computer Communication Review}}
  \bibinfo{volume}{44}, \bibinfo{number}{5} (\bibinfo{year}{2014}),
  \bibinfo{pages}{33--38}.
\newblock


\bibitem[Norrman et~al\mbox{.}(2016)]%
        {norrman2016protecting}
\bibfield{author}{\bibinfo{person}{Karl Norrman}, \bibinfo{person}{Mats
  N{\"a}slund}, {and} \bibinfo{person}{Elena Dubrova}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Protecting IMSI and user privacy in 5G networks}}.
  In \bibinfo{booktitle}{\emph{Proceedings of the 9th EAI international
  conference on mobile multimedia communications}}. \bibinfo{pages}{159--166}.
\newblock


\bibitem[Olimid and Mj{\o}lsnes(2017)]%
        {olimid2017lowcost}
\bibfield{author}{\bibinfo{person}{Ruxandra~F Olimid} {and}
  \bibinfo{person}{Stig~F Mj{\o}lsnes}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{On LowCost Privacy Exposure Attacks in LTE Mobile
  Communication}}.
\newblock \bibinfo{journal}{\emph{Proceedings of the Romanian Academy Series
  AMathematics Physics Technical Sciences Information Science}}
  \bibinfo{volume}{18} (\bibinfo{year}{2017}), \bibinfo{pages}{361--370}.
\newblock


\bibitem[Paget(2010)]%
        {paget2010practical}
\bibfield{author}{\bibinfo{person}{Chris Paget}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{{Practical cellphone spying}}.
\newblock \bibinfo{journal}{\emph{Def Con}}  \bibinfo{volume}{18}
  (\bibinfo{year}{2010}).
\newblock


\bibitem[Palam{\`a} et~al\mbox{.}(2021)]%
        {palama2021imsi}
\bibfield{author}{\bibinfo{person}{Ivan Palam{\`a}}, \bibinfo{person}{Francesco
  Gringoli}, \bibinfo{person}{Giuseppe Bianchi}, {and} \bibinfo{person}{Nicola
  Blefari-Melazzi}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{IMSI Catchers in the wild: A real world 4G/5G
  assessment}}.
\newblock \bibinfo{journal}{\emph{Computer Networks}}  \bibinfo{volume}{194}
  (\bibinfo{year}{2021}), \bibinfo{pages}{108137}.
\newblock


\bibitem[Parcu et~al\mbox{.}(2023)]%
        {5G_stats}
\bibfield{author}{\bibinfo{person}{Pier~Luigi Parcu},
  \bibinfo{person}{Anna~Renata Pisarkiewicz}, \bibinfo{person}{Chiara
  Carrozza}, {and} \bibinfo{person}{Niccolò Innocenti}.}
  \bibinfo{year}{2023}\natexlab{}.
\newblock \showarticletitle{The future of 5G and beyond: Leadership, deployment
  and European policies}.
\newblock \bibinfo{journal}{\emph{Telecommunications Policy}}
  \bibinfo{volume}{47}, \bibinfo{number}{9} (\bibinfo{year}{2023}),
  \bibinfo{pages}{102622}.
\newblock
\showISSN{0308-5961}
\urldef\tempurl%
\url{https://doi.org/10.1016/j.telpol.2023.102622}
\showDOI{\tempurl}


\bibitem[Park et~al\mbox{.}(2022)]%
        {park2022doltest}
\bibfield{author}{\bibinfo{person}{CheolJun Park}, \bibinfo{person}{Sangwook
  Bae}, \bibinfo{person}{BeomSeok Oh}, \bibinfo{person}{Jiho Lee},
  \bibinfo{person}{Eunkyu Lee}, \bibinfo{person}{Insu Yun}, {and}
  \bibinfo{person}{Yongdae Kim}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{$\{$DoLTEst$\}$: In-depth Downlink Negative Testing
  Framework for $\{$LTE$\}$ Devices}. In \bibinfo{booktitle}{\emph{31st USENIX
  Security Symposium (USENIX Security 22)}}. \bibinfo{pages}{1325--1342}.
\newblock


\bibitem[Park et~al\mbox{.}(2021)]%
        {park20215g}
\bibfield{author}{\bibinfo{person}{Seongmin Park}, \bibinfo{person}{Daeun Kim},
  \bibinfo{person}{Youngkwon Park}, \bibinfo{person}{Hyungjin Cho},
  \bibinfo{person}{Dowon Kim}, {and} \bibinfo{person}{Sungmoon Kwon}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{5G security threat assessment in real networks}}.
\newblock \bibinfo{journal}{\emph{Sensors}} \bibinfo{volume}{21},
  \bibinfo{number}{16} (\bibinfo{year}{2021}), \bibinfo{pages}{5524}.
\newblock


\bibitem[Park et~al\mbox{.}(2019)]%
        {park2019anatomy}
\bibfield{author}{\bibinfo{person}{Shinjo Park}, \bibinfo{person}{Altaf Shaik},
  \bibinfo{person}{Ravishankar Borgaonkar}, {and} \bibinfo{person}{Jean-Pierre
  Seifert}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{Anatomy of commercial IMSI catchers and
  detectors}}. In \bibinfo{booktitle}{\emph{Proceedings of the 18th ACM
  Workshop on Privacy in the Electronic Society}}. \bibinfo{pages}{74--86}.
\newblock


\bibitem[RCRWirelessNews(2024)]%
        {5gsa}
\bibfield{author}{\bibinfo{person}{RCRWirelessNews}.}
  \bibinfo{year}{2024}\natexlab{}.
\newblock \bibinfo{title}{{2024 will be a catalyst for accelerating 5G
  Standalone/5G Core deployments}}.
\newblock
  \bibinfo{howpublished}{\url{https://www.rcrwireless.com/20240130/opinion/readerforum/2024-will-be-a-catalyst-for-accelerating-5g-standalone-5g-core-deployments-reader-forum}}.
\newblock
\newblock
\shownote{Accessed: 2024-02}.


\bibitem[Rupprecht et~al\mbox{.}(2018)]%
        {rupprecht2018security}
\bibfield{author}{\bibinfo{person}{David Rupprecht}, \bibinfo{person}{Adrian
  Dabrowski}, \bibinfo{person}{Thorsten Holz}, \bibinfo{person}{Edgar Weippl},
  {and} \bibinfo{person}{Christina P{\"o}pper}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{On security research towards future mobile network
  generations}}.
\newblock \bibinfo{journal}{\emph{IEEE Communications Surveys \& Tutorials}}
  \bibinfo{volume}{20}, \bibinfo{number}{3} (\bibinfo{year}{2018}),
  \bibinfo{pages}{2518--2542}.
\newblock


\bibitem[Rupprecht et~al\mbox{.}(2019)]%
        {rupprecht2019breaking}
\bibfield{author}{\bibinfo{person}{David Rupprecht}, \bibinfo{person}{Katharina
  Kohls}, \bibinfo{person}{Thorsten Holz}, {and} \bibinfo{person}{Christina
  P{\"o}pper}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{Breaking LTE on layer two}}. In
  \bibinfo{booktitle}{\emph{2019 IEEE Symposium on Security and Privacy (SP)}}.
  IEEE, \bibinfo{pages}{1121--1136}.
\newblock


\bibitem[Rupprecht et~al\mbox{.}(2020)]%
        {rupprecht2020call}
\bibfield{author}{\bibinfo{person}{David Rupprecht}, \bibinfo{person}{Katharina
  Kohls}, \bibinfo{person}{Thorsten Holz}, {and} \bibinfo{person}{Christina
  P{\"o}pper}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{{Call me maybe: Eavesdropping encrypted $\{$LTE$\}$
  calls with $\{$ReVoLTE$\}$}}. In \bibinfo{booktitle}{\emph{29th USENIX
  security symposium (USENIX security 20)}}. \bibinfo{pages}{73--88}.
\newblock


\bibitem[Shaik et~al\mbox{.}(2015)]%
        {shaik2015practical}
\bibfield{author}{\bibinfo{person}{Altaf Shaik}, \bibinfo{person}{Ravishankar
  Borgaonkar}, \bibinfo{person}{N Asokan}, \bibinfo{person}{Valtteri Niemi},
  {and} \bibinfo{person}{Jean-Pierre Seifert}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{{Practical attacks against privacy and availability
  in 4G/LTE mobile communication systems}}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1510.07563}}
  (\bibinfo{year}{2015}).
\newblock


\bibitem[Shaik et~al\mbox{.}(2019)]%
        {shaik2019new}
\bibfield{author}{\bibinfo{person}{Altaf Shaik}, \bibinfo{person}{Ravishankar
  Borgaonkar}, \bibinfo{person}{Shinjo Park}, {and}
  \bibinfo{person}{Jean-Pierre Seifert}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{New vulnerabilities in 4G and 5G cellular access
  network protocols: exposing device capabilities}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 12th Conference on Security and
  Privacy in Wireless and Mobile Networks}}. \bibinfo{pages}{221--231}.
\newblock


\bibitem[Strobel(2007)]%
        {strobel2007imsi}
\bibfield{author}{\bibinfo{person}{Daehyun Strobel}.}
  \bibinfo{year}{2007}\natexlab{}.
\newblock \showarticletitle{{IMSI catcher}}.
\newblock \bibinfo{journal}{\emph{Chair for Communication Security,
  Ruhr-Universit{\"a}t Bochum}}  \bibinfo{volume}{14} (\bibinfo{year}{2007}).
\newblock


\bibitem[Van Den~Broek et~al\mbox{.}(2015)]%
        {van2015defeating}
\bibfield{author}{\bibinfo{person}{Fabian Van Den~Broek}, \bibinfo{person}{Roel
  Verdult}, {and} \bibinfo{person}{Joeri De~Ruiter}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{{Defeating IMSI catchers}}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 22Nd ACM SIGSAC Conference on
  Computer and Communications Security}}. \bibinfo{pages}{340--351}.
\newblock


\bibitem[Wang et~al\mbox{.}(2021)]%
        {wang2021privacy}
\bibfield{author}{\bibinfo{person}{Yuchen Wang}, \bibinfo{person}{Zhenfeng
  Zhang}, {and} \bibinfo{person}{Yongquan Xie}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{$\{$Privacy-Preserving$\}$ and
  $\{$Standard-Compatible$\}$$\{$AKA$\}$ Protocol for 5G}. In
  \bibinfo{booktitle}{\emph{30th USENIX Security Symposium (USENIX Security
  21)}}. \bibinfo{pages}{3595--3612}.
\newblock


\bibitem[Wani et~al\mbox{.}(2024)]%
        {wani2024security}
\bibfield{author}{\bibinfo{person}{Mohamad~Saalim Wani},
  \bibinfo{person}{Michael Rademacher}, \bibinfo{person}{Thorsten Horstmann},
  {and} \bibinfo{person}{Mathias Kretschmer}.} \bibinfo{year}{2024}\natexlab{}.
\newblock \showarticletitle{{Security Vulnerabilities in 5G Non-Stand-Alone
  Networks: A Systematic Analysis and Attack Taxonomy}}.
\newblock \bibinfo{journal}{\emph{Journal of Cybersecurity and Privacy}}
  \bibinfo{volume}{4}, \bibinfo{number}{1} (\bibinfo{year}{2024}),
  \bibinfo{pages}{23--40}.
\newblock


\bibitem[Yang et~al\mbox{.}(2019)]%
        {yang2019hiding}
\bibfield{author}{\bibinfo{person}{Hojoon Yang}, \bibinfo{person}{Sangwook
  Bae}, \bibinfo{person}{Mincheol Son}, \bibinfo{person}{Hongil Kim},
  \bibinfo{person}{Song~Min Kim}, {and} \bibinfo{person}{Yongdae Kim}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{{Hiding in plain signal: Physical signal
  overshadowing attack on $\{$LTE$\}$}}. In \bibinfo{booktitle}{\emph{28th
  USENIX Security Symposium (USENIX Security 19)}}. \bibinfo{pages}{55--72}.
\newblock


\bibitem[Yu et~al\mbox{.}(2021)]%
        {yu2021improving}
\bibfield{author}{\bibinfo{person}{Chuan Yu}, \bibinfo{person}{Shuhui Chen},
  \bibinfo{person}{Fei Wang}, {and} \bibinfo{person}{Ziling Wei}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{{Improving 4G/5G air interface security: A survey
  of existing attacks on different LTE layers}}.
\newblock \bibinfo{journal}{\emph{Computer Networks}}  \bibinfo{volume}{201}
  (\bibinfo{year}{2021}), \bibinfo{pages}{108532}.
\newblock


\bibitem[Zhang and Fang(2005)]%
        {zhang2005security}
\bibfield{author}{\bibinfo{person}{Muxiang Zhang} {and}
  \bibinfo{person}{Yuguang Fang}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{{Security analysis and enhancements of 3GPP
  authentication and key agreement protocol}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on wireless
  communications}} \bibinfo{volume}{4}, \bibinfo{number}{2}
  (\bibinfo{year}{2005}), \bibinfo{pages}{734--742}.
\newblock


\end{thebibliography}

